VaB-AL: Incorporating Class Imbalance and Difficulty with Variational Bayes for Active Learning

Active Learning for discriminative models has largely been studied with the focus on individual samples, with less emphasis on how classes are distributed or which classes are hard to deal with. In this work, we show that this is harmful. We propose a method based on the Bayes' rule, that can naturally incorporate class imbalance into the Active Learning framework. We derive that three terms should be considered together when estimating the probability of a classifier making a mistake for a given sample; i) probability of mislabelling a class, ii) likelihood of the data given a predicted class, and iii) the prior probability on the abundance of a predicted class. Implementing these terms requires a generative model and an intractable likelihood estimation. Therefore, we train a Variational Auto Encoder (VAE) for this purpose. To further tie the VAE with the classifier and facilitate VAE training, we use the classifiers' deep feature representations as input to the VAE. By considering all three probabilities, among them especially the data imbalance, we can substantially improve the potential of existing methods under limited data budget. We show that our method can be applied to classification tasks on multiple different datasets -- including one that is a real-world dataset with heavy data imbalance -- significantly outperforming the state of the art.

==> figs/ablation/item.tex <==
\begin{figure*}[t]
\centering
\subfigure[Results with varying budget sizes.]{\includegraphics[width=0.45\linewidth]{figs/ablation/ablation_budget2}}
\subfigure[Results with varying $\lambda$.]{\includegraphics[width=0.45\linewidth]{figs/ablation/ablation_lambda2}}
\caption{Results of ablation tests on \textit{dominant} CIFAR-10.}
\label{fig:ablation_graph}
\end{figure*}

==> figs/correlation/item.tex <==
\begin{minipage}{0.48\textwidth}
% \begin{figure}[H]
\centering
\includegraphics[width=0.9\textwidth]{figs/correlation/corr_fullCIFAR10.pdf}
\vspace{-1em}
\caption{\textbf{Correlation between the class-wise accuracy and the class-wise sample sizes -- }We show a scatter plot of the accuracy of different classes vs the number of sample extracted for each class.
For classes with high accuracy, our method samples less of them, focusing on the hard ones.}
\label{fig:fullCIFAR10_correlation}
% \end{figure}
\end{minipage}

==> figs/latent/item.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth,height=6cm]{figs/dummy_image.png}
\caption{{\bf Latent embedding example -- }An example of the learned latent embeddings with the regularizatoin for the MNIST dataset.
% \TODO{some teaser showing that we use label correctness, likelihood, prior from labeled pool to estimate on the unlabeled pool?}
\TODO{Figure, Improve caption}
\JW{Regularized VAE의 Latent Feature 특성을 Empirical하게 보여주기. (각 split feature에서 서로 다른 클래스의 샘플들이 0에 가까이 위치하는 모습)}
}
\label{fig:latent}
\end{figure}

==> figs/new_result/dominantFig.tex <==
\begin{figure*}[t]
\centering
\subfigure[NEU dataset]{\includegraphics[width=0.32\linewidth]{figs/new_result/NEU_CLS_ACC}}
\subfigure[\textit{dominant} CIFAR-10]{\includegraphics[width=0.32\linewidth]{figs/new_result/DOMINANT_CIFAR10_ACC.pdf}}
\subfigure[\textit{dominant} CIFAR-100]{\includegraphics[width=0.32\linewidth]{figs/new_result/DOMINANT_CIFAR100_ACC.pdf}}
\vspace{-1mm}
\caption{Results for the dominant datasets. }
\vspace{-5mm}
\label{fig:dominantDatasets}
\end{figure*}

==> figs/new_result/fullFig.tex <==
\begin{figure*}[t]
\centering
\subfigure[\textit{Rare} CIFAR-10]{\includegraphics[width=0.32\linewidth]{figs/new_result/RARE_CIFAR10_ACC.pdf}}
\subfigure[\textit{Full} CIFAR-10]{\includegraphics[width=0.32\linewidth]{figs/new_result/FULL_CIFAR10_ACC.pdf}}
\subfigure[\textit{Full} CIFAR-100]{\includegraphics[width=0.32\linewidth]{figs/new_result/FULL_CIFAR100_ACC.pdf}}
\vspace{-1mm}
\caption{Results for the rare and full datasets.}
\vspace{-4mm}
\label{fig:fullDatasets}
\end{figure*}

==> figs/result/dominantCIFAR10.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figs/result/dominantCIFAR10}
\caption{Results for the \textit{dominant} variants of CIFAR-10.}
\label{fig:dominantCIFAR10}
\end{figure}

==> figs/result/dominantCIFAR100.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figs/result/dominantCIFAR100}
\caption{Results for the \textit{dominant} variants of CIFAR-100.}
\label{fig:dominantCIFAR100}
\end{figure}

==> figs/result/dominantFig.tex <==
\begin{figure*}[t]
\centering
\subfigure[NEU dataset]{\includegraphics[width=0.32\linewidth]{figs/result/fullNEU}}
\subfigure[\textit{dominant} CIFAR-10]{\includegraphics[width=0.32\linewidth]{figs/result/dominantCIFAR10}}
\subfigure[\textit{dominant} CIFAR-100]{\includegraphics[width=0.32\linewidth]{figs/result/dominantCIFAR100}}
\caption{Results for the dominant datasets. \hj{Fig3하고 4 그래프는 아래위로 조금 더 납작한 그림 있나? space를 더 줄여하 하는데..}}
\label{fig:dominantDatasets}
\end{figure*}

==> figs/result/fullCIFAR10.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figs/result/fullCIFAR10}
\caption{Results for the full CIFAR-10 dataset.}
\label{fig:fullCIFAR10}
\end{figure}

==> figs/result/fullCIFAR100.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figs/result/fullCIFAR100}
\caption{Results for the full CIFAR-100 dataset.}
\label{fig:fullCIFAR100}
\end{figure}

==> figs/result/fullFig.tex <==
\begin{figure*}[t]
\centering
\subfigure[\textit{Rare} CIFAR-10]{\includegraphics[width=0.32\linewidth]{figs/result/rareCIFAR10}}
\subfigure[\textit{Full} CIFAR-10]{\includegraphics[width=0.32\linewidth]{figs/result/fullCIFAR10}}
\subfigure[\textit{Full} CIFAR-100]{\includegraphics[width=0.32\linewidth]{figs/result/fullCIFAR100}}
\caption{Results for the rare and full datasets.}
\label{fig:fullDatasets}
\end{figure*}

==> figs/result/fullNEU.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figs/result/fullNEU}
\caption{Results for the NEU dataset.
% We report results for the NEU dataset by running five active sampling rounds, where each round we take 250 samples from the unlabelled pool. number of samples, allowing faster convergence.
% Our method performs best, especially with less number of samples, allowing faster convergence.
}
\label{fig:fullNEU}
\end{figure}

==> figs/result/rareCIFAR10.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figs/result/rareCIFAR10}
\caption{Results for the \textit{rare} variants of CIFAR-10.}
\label{fig:rareCIFAR10}
\end{figure}

==> old/3-Framework0.tex <==
\section{Method}
\label{sec:method}

At every step of active learning, we divide the entire training data by three pools.
At first, the \textit{unlabeled pool} ($\mathcal{P}^o$) contains all the samples that are not labeled yet.
The \textit{labeled pool} ($\mathcal{P}$) consists of the other samples labeled by the users.
We further divide $\mathcal{P}$ by two pools: a labeled pool for VAE training ($\mathcal{P}_v$) and a labeled pool for uncertainty estimation ($\mathcal{P}_e$).
Thus, $\mathcal{P}=\mathcal{P}_v \bigcup \mathcal{P}_e$ is always satisfied, and $\mathcal{P}_v$ and $\mathcal{P}_e$ are utilized for training the VAE module and estimating the posterior probability, respectively.
%The labeled pool for VAE training contains most of the samples in the labeled pool, while all the remaining samples are included in the labeled pool for the uncertainty estimation, so .
%the naive approach that selects the ambiguous samples to balance the class-wise sample numbers is contradicted.


\begin{algorithm}[t]
\small
    \label{algorithm}
    \caption{Posterior Active Learning}
    Input: $\mathcal{P^o}$, $\mathcal{P}$, $N_s$\\
    
    \While{not at the maximum sampling iteration}{
        Train $\mathcal{M}$ using $\mathcal{P}$ and its own loss\\
        Freeze $\mathcal{M}$\\
        Divide $\mathcal{P}$ by $\mathcal{P}_v$ and $\mathcal{P}_e$
        Train the VAE module using $\mathcal{P}_v$ and Eq.~\ref{eq:vaeLoss}\\
        Estimate the label uncertainty probability using Eq.~\ref{eq:labelUncertaintyProb}\\
        Estimate the prior probability using Eq.~\ref{eq:prior}\\
        Estimate the likelihood probability using Eq.~\ref{eq:likelihood}\\
        Estimate the posterior uncertainty using Eq.~\ref{eq:posteriorUncertainty}\\
        $\mathbf{X}$ $\leftarrow$ Sample $N_s$ samples with the highest uncertainty\\
        $\mathcal{P^o}$ $\leftarrow$ $\mathcal{P^o}$ - $\mathbf{X}$\\
        $\mathcal{P}$ $\leftarrow$ $\mathcal{P}$ $\bigcup$ $\mathbf{X}$\\
    }
    \normalsize
\end{algorithm}


\subsection{Overall Structure}
As shown in Fig.~\jw{figure}, the entire architecture of the proposed algorithm contains two sub-networks: one baseline network and one VAE.
The structure of the baseline network follows the original architecture used by the target algorithm for the active learning, and the VAE is fed by the multiple features from the baseline network.
%We denote the baseline network and the VAE by $\mathcal{M}$ and $\mathcal{V}$, respectively.

At the initial state where every training sample is included in $\mathcal{P}^o$, the defined number ($N_s$) of samples are randomly selected for the initial training.
After the initial samples are labeled by the users, the samples are excluded from $\mathcal{P}^o$ and added into $\mathcal{P}$ with the labels.
Then, by using the updated $\mathcal{P}$, we train the baseline network by the original training method of the target task.
After freezing the trained baseline network, we train the VAE to represent both of the overall and class-wise distributions by $\mathcal{P}$ and $\mathcal{P}_v$.
%The training scheme drives the latent space of VAE to represent the overall and class-wise distributions simultaneously.
From the trained distributions of the VAE and $\mathcal{P}_e$, we estimate the posterior uncertainty of every sample in $\mathcal{P}^o$, and the $N_s$ unlabeled samples with the highest posterior uncertainty are chosen for the user labeling.
Finally, the labeled samples are moved from $\mathcal{P}^o$ to $\mathcal{P}$, and then we repeat the training of the baseline network by using the updated $\mathcal{P}$.
The details of the procedures are summarized in Algorithm~\ref{algorithm}.


==> old/3-Framework1.tex <==
\subsection{VAE Module}
The VAE utilizes the multiple features of the baseline network as its input, and thus the size of the VAE can be much smaller than that of the baseline network.
To represent the overall and class-wise feature distributions in the latent space of the VAE, we split the dimensions of the latent features in the VAE according to the number of classes.
Then, while the entire latent feature depicts the overall feature distribution, the class-wise feature distribution can be found when we consider only the split latent features.
Since the latent features are hypothetically divided, the architecture of the VAE is equivalent with the conventional VAE, but the training scheme is novel to train the class-wise feature distribution.
%The latent space of the VAE module represents the overall feature distribution as the conventional VAE.
%In the while, the VAE is trained to represent the class-wise feature distribution as well.

\subsubsection{Architecture}
The raw features extracted from the baseline network are pre-processed before being fed into the VAE.
When the extracted feature is a convolution feature, we reduce the feature size by applying a global average pooling layer (GAP).
Then, each of the features is respectively normalized by a batch normalization layer to align the various feature distributions from the multiple layers.
%After reducing the feature size, each of the a batch normalization is applied to normalize the various distribution from the multiple layers.
Finally, the normalized features are fed respectively into the fully-connected layers, and then the feature vector concatenated by the outputs of the fully-connected layers is fed into the input of the VAE.
Then, we denote the feature extraction and the pre-processing processes by $\mathcal{H}(\bullet)$ as following:
\begin{equation}
    \mathbf{h}^{(i)} = \mathcal{H} (\mathbf{x}^{(i)}),
\end{equation}
where $\mathbf{h}^{(i)}$ is the input of the VAE when the image sample $\mathbf{x}^{(i)}$ is given.

As the conventional VAE, the VAE module consists of one probabilistic encoder and one decoder that are denoted by $q_{\phi}(\mathbf{z}|\mathbf{h})$ and $p_{\theta}(\mathbf{h}|\mathbf{z})$, respectively.
Both of the encoder and decoder is composed of multiple fully-connected layers followed by ReLU.
Then, the random variable $\tilde{\mathbf{z}}\sim q_{\phi}(\mathbf{z}|\mathbf{h})$ can be reformulated by using an auxiliary noise variable $\mathbf{\epsilon}$ as following:
\begin{equation}
    \tilde{\mathbf{z}}^{(i,l)} = g_{\phi}(\epsilon^{(l)}, \mathbf{h}^{(i)}) \,\,\,\,\,\,\,\,with\,\,\,\epsilon^{(l)} \sim \mathcal{N}(0,1),
\end{equation}
where $\mathcal{N}(\mu,\sigma^2)$ is a Gaussian probability distribution with a average $\mu$ and a standard deviation $\sigma$.

From the sampled $\tilde{\mathbf{z}}$, the class-wise response probability $\mathbf{r}$ is estimated by the softmax probability as:
\begin{equation}
\begin{aligned}
    \tilde{\mathbf{r}} &= softmax \bigg(\Big[\sum_{j\in C_1} -z_j^2, \sum_{j\in C_2} -z_j^2, \dots, \sum_{j\in C_{N_c}} -z_j^2\Big]^T\bigg),
\end{aligned}
\end{equation}
where $N_c$ means the number of classes, $z_j$ is the $j$-th dimension value of $\mathbf{z}$, and $C_n$ is a set of indices for the split dimensions of $\mathbf{z}$ that represent the $n$-th class.
\jw{
Thus, in the class-wise feature distribution, the samples of the target classes are located near $0$ on the split dimensions that represent the target class.
Then, the samples of the other classes are placed far from $0$.
 - 다시 쓰기}

\jw{여기서 이렇게 학습된 latent feature의 특성을 보여주면 좋을듯. 각 클래스별 latent vector들을 보면 특정 클래스의 sample들이 0에 뭉쳐있고 나머지는 외부에 배치. 혹은 2-D로 보여주는 것도 재밌는 방법이 될수도 있음.}


\subsubsection{Training Method}
We define the samples from $\mathcal{P}_v$ by $\{\mathbf{x}_v^{(i)}\}$ and the samples from $\mathcal{P}^o$ by $\{\mathbf{x}_o^{(i)}\}$.
After finishing the training of the baseline network, the weights of the baseline network are frozen to avoid the degradation of its performance.
Thus, when the VAE is trained, only the preprocessing layers and the layers of the VAE modules are updated.
As a result, when the users want to stop the active learning, the baseline network can be served directly as the final model without any additional training sequence.

To let the latent features represent the overall and class-wise feature distribution simultaneously, we define the loss $\mathcal{L}$ by:
\begin{equation}\label{eq:vaeloss}
    \mathcal{L} = \mathcal{L}_{overall} + \lambda_c \mathcal{L}_{class},
\end{equation}
where $\mathcal{L}_{overall}$ and $\mathcal{L}_{class}$ denotes the losses for the overall and class-wise feature distribution, respectively, with $\lambda_c$ that controls the ratio of the two losses.

The overall feature distribution is trained by using the loss terms that were proposed in~\jw{VAE refer}.
Thus,
\begin{equation} \label{eq:vaeLoss}
    \mathcal{L}_{overall} = \mathbb{E}[\log p_{\theta}(\mathbf{h}|\mathbf{z})] - \mathbf{D}_{KL}\big(q_{\phi}(\mathbf{z}|\mathbf{h})\parallel p(\mathbf{z})\big).
\end{equation}
Since $\mathcal{L}_{overall}$ can be estimated even with the unlabeled data, every sample from both of $\mathcal{P}_v$ and $\mathcal{P}^o$ is utilized for learning the overall feature distribution.
$p(\mathbf{z})$ is the prior that is chosen by a unit Gaussian ($\mathcal{N}(0,1)$).
Referred by~\jw{VAE refer}, we use the reparameterization trick to calculate the gradients from the sampling-based loss.

Like $\mathcal{L}_{overall}$ considering all the training data, $\mathcal{L}_{class}$ contains the two loss terms acquired by $\mathcal{P}_v$ and $\mathcal{P}^o$, respectively.
\begin{equation}
    \mathcal{L}_{class} = - \sum_{\mathbf{x}^{(i)}_v \in \mathcal{P}_v} \mathbf{y}^{(i)}_v \log \tilde{\mathbf{r}}^{(i)}_v - \sum_{\mathbf{x}^{(i)}_o \in \mathcal{P}_o} \tilde{\mathbf{r}}^{(i)}_o \log \tilde{\mathbf{r}}^{(i)}_o,
\end{equation}
where $\mathbf{y}^{(i)}_v$ is a one-hot vector for the labels paired by $\mathbf{x}^{(i)}_v$.
Among the two loss terms in $\mathcal{L}_{class}$, the first loss term is the conventional cross-entropy loss for the labeled samples, while the second loss term drives the unlabeled samples to be associated one of the multiple classes by the marginal entropy loss.

To update the VAE, we build a mini-batch with $N_b$ samples by randomly extracting $N_b/2$ samples from $\mathcal{P}_v$ and the other samples from $\mathcal{P}^o$.
The weights of the VAE are updated by Adam Optimizer~\jw{refer}.

% For the labeled samples, the class-wise response is updated by the supervised learning scheme.
% \begin{equation}
%     L_{class1} = \sum_{i=1}^{N_b/2} -\mathbf{y} \log \mathbf{p}(\mathbf{x}_i).
% \end{equation}

% Assuming that the unlabeled samples should be included in one of the multiple classes, we consider the unlabeled class for the class-wise distribution by a marginal entropy loss as:
% \begin{equation}
%     L_{class2} = \sum_{i=1}^{N_b/2} -\mathbf{p}(\mathbf{x}^o_i) \log \mathbf{p}(\mathbf{x}^o_i).
% \end{equation}

% In addition, we define the classifier based on the latent space of the trained VAE by $D$ that is:
% \begin{equation}
%     D(f(x, \epsilon)) = \arg \max [r_1, r_2, ..., r_{N_c}].
% \end{equation}

% The loss term to train the VAE module is calcumated by summing all the loss terms at every iteration.
% We use Adam Optimizer~\jw{refer} to update the VAE module.





==> old/3-Framework2.tex <==
\subsection{Class-wise Sampling Number Estimation}
Initial sampling number estimation (assume all the predicted labels are correct)

Sampling number refinement (consider the class간의 prediction ambiguity)


\subsubsection{Initial Sampling Number Estimation}
Introduction of Water-filling algorithm

0. $S={0,...,N_c}$

1. iterate for $i$-th class maximum sample number, $S \leftarrow S - \{index of i\}$

2. if $ \{index of i\}-th class sample number \times #(S) - \sum_{j \in S} j-th class sample number < N_{sampling}$

2-1. $eta = \frac{N_{sampling} - \sum_{j \in S} j-th class sample number}{N_c - i + 1} + $ $i$-th class maximum sample number

2-2. $j$-th result $=$ $eta - j-th class sample number$ for $S$, otherwise 0

2-3. break


\subsubsection{Sampling Number Refinement?}
Sampling Number Refinement를 위한 기본 식 정의

Posterior probability definition ($p(y_n|\widehat{y_m})$)

여기서 Initial sampling number가 ideal case이고, uncertainty?를 기반으로 계산한 sampling number를 얻고자 할 때, 아래와 같이 정의
\begin{equation}
    \mathbf{N} = \mathbf{P} \mathbf{\widehat{N}}
\end{equation}

\begin{equation}
    \begin{aligned}
        \mathbf{P} &= \mathcal{R}^{N_c\times N_c}\\
        \mathbf{P}_{n, m} &= p(y_n|\widehat{y_m})
    \end{aligned}
\end{equation}


2. Bayes rule-based posterior probability estimation
\begin{equation}
    p(y_n|\widehat{y_m}) = \frac{p(y_n) p(\widehat{y_m}|y_n)}{\sum_{n=1}^{N_c} p(\widehat{y_m}|y_n)}
\end{equation}

3. Real label prior probability estimation ($p(y_n)$): Approximated by the class-wise sample ratio at the initial random sampling.

4. Likelihood probability estimation ($p(\widehat{y_m}|y_n)$): Estimated by predicting the labels for labeled data''.
: N times sampling > probability estimation


이 후 $\mathbf{\widehat{N}}$을 추정하기 위해 Convex optimization 풀기.

5. Convex optimization for estimating the refined sampling number

\begin{equation}
    \mathbf{N} = \mathbf{P} \mathbf{\widehat{N}}
\end{equation}
s.t. sum($\widehat{N}$)=$N_{sampling}$, \widehat{N} is integer

\begin{equation}
    E = ||\mathbf{N}_{init} - \mathbf{P} \widehat{\mathbf{N}}||_2^2 + \lambda||\mathbf{N}_{init} - \widehat{\mathbf{N}}||_2^2 + \lambda_p (\mathbf{N}_{sampling} - \sum\widehat{\mathbf{N}})^2
\end{equation}

5-1. Loss term 1: $(N - P * \widehat{N})^2$. 추정되는 Sampling number개수가 Real 기준 개수와 유사해지도록 Posterior probability 곱.

5-2. Loss term 2: $(N - \widehat{N})^2$. 다만, 추정되는 sampling number와 Real sampling number가 너무 크게 차이나지 않게. 만약 없으면 1번 loss term에 의해 특정 클래스로 추정되는 샘플들만 선택하려고 하는 경향이 매우 강해짐. (특히 dominant class 상황일 때 dominant class를 선택하지 않으려는 특성이 강한데 이로인해 dominant class로 잘못 추정될 가능성이 가장 적은 class의 sample만 선택하도록 최적화 결과가 나오는 경우 많음.)

5-3. Penalty term 2: $\lambda_p(\sum\widehat{N} - N_{sampling})^2$ 클래스별 샘플링하는 샘플의 총합은 우리가 원하는 전체 샘플링하는 샘플의 개수와 같아야 함. 원래는 constraint지만 penalty term으로 넣어서 relaxation.

5-4. Optimization: Non-negative Least Square Optimization 알고리즘 적용. 개수는 Integer이기 때문에 Integer programming 등을 이용해야하지만, 효율적인 계산을 위해 Interger를 일반 Float으로 Relaxation시켜 계산한 뒤, Round시켜 최종 결과값 추정. 만약 round로 인해 총합이 사용자가 원하는 sample개수와 다르거나 원하는 sample 개수만큼의 sample이 해당 클래스에 존재하지 않는 경우, 가장 앞선 클래스부터 더하거나 하나씩 빼서 개수를 맞춘다.

==> old/3-Framework3.tex <==
\subsection{Active Sampling Algorithm}
Using the trained VAE, we estimate the posterior uncertainty of the unlabeled samples $\bx_o^{(i)}$ from $\calP^o$.
At first, we define the uncertainty of the training sample $\bx$ by:
\begin{equation}
    P( \by \neq \widehat{\by} | \bx ),
\end{equation}
where $\by$ and $\widehat{\by}$ are the real label and the predicted label of $\bx$, respectively.
$\widehat{\by}$ is predicted by the class-wise feature distribution trained in the VAE as:
\begin{equation}
    \widehat{\by} = \arg \max [\tilde{r}_1, \tilde{r}_2, \dots, \tilde{r}_{N_c}].
\end{equation}

Then, we derive the posterior uncertainty as following:
\begin{equation}\label{eq:posteriorUncertainty}
    \begin{aligned}
        P(\by \neq \widehat{\by} | \bx)
        &= 1 - P(\by = \widehat{\by} | \bx)\\
        &= 1 - \sum_{n=1}^{N_c} P(\by_n, \widehat{\by}_n | \bx),
    \end{aligned}
\end{equation}
where $\by_n$ and $\widehat{\by}_n$ mean $\by=n$ and $\widehat{\by}=n$, respectively.
Unfortunately, it is infeasible to estimate the posterior probability of $P(\by_n, \widehat{\by}_n | \bx)$ directly, so we reformulate it through Bayes rule as:
\begin{equation}
    \begin{aligned}
        P(\by_n, \widehat{\by}_n | \bx) 
        = P(\by_n | \widehat{\by}_n, \bx) P(\bx | \widehat{\by}_n) P(\widehat{\by}_n) / P(\bx).
    \end{aligned}
\end{equation}
We denote $P(\by_n | \widehat{\by}_n, \bx)$, $P(\bx | \widehat{\by}_n)$, and $P(\widehat{\by}_n)$ by a \textit{label uncertainty}, a \textit{likelihood}, and a \textit{prior}, respectively.
\ky{Here, $P(\by_n | \widehat{\by}_n, \bx)$ again involves $\by$ and $\bx$, which cannot be evaluated until we observe the label.
Therefore, we instead do an informed guess, by ignoring $\bx$ and approximating with $P(\by_n | \widehat{\by}_n)$, in other words, relying on our current estimate of our label.
We therefore write
}

% However, even after the reformulation, the label uncertainty for the unlabeled samples cannot be estimated yet since the real labels of the unlabeled samples are unknown. 
% Thus, we assume that the real label of the unlabeled sample has a uniform distribution. \jw{확률론? 슈뢰딩거의 고양이? ㅋㅋㅋ} 
% \KY{Here, $P(\by_n | \widehat{\by}_n)$ here is a posterior probabilty that we cannot make sense of until}
% Based on the assumption, we ignore the given condition $x$ in the label uncertainty (i.e. $P(\by_n | \widehat{\by}_n, \bx) \approx P(\by_n | \widehat{\by}_n)$), and then we can derive the posterior probability as:
\begin{equation}
    \begin{aligned}
        P(\by\neq\widehat{\by} | \bx) \propto C - \sum_{n=1}^{N_c} P(\by_n | \widehat{\by}_n) P(\bx | \widehat{\by}_n) P(\widehat{\by}_n),
    \end{aligned}
\end{equation}
when $P(\bx)=C$ follows the uniform distribution.

%\jw{앞서 언급할 Assumption에 대한 간단한 Toy 결과 보여주기?}
%\jw{여기서 Sampling할 때 세개의 각 term들의 역할에 대해 간단하게 짚어줘야할 듯.}
%\jw{Label uncertainty: 부정확한 라벨로 추정될 확률이 높은 샘플의 경우 선택 가능성 높아짐. 즉, 라벨에 따라서 데이터가 더 필요한 경우 샘플링 가능성 업}
%\jw{Prior: 샘플 개수가 적어 샘플링 가능성이 낮은 경우 prior를 기반으로 클래스 별 개수에 상관없이 샘플링 가능성을 비슷하게 하도록 보정}
%\jw{Likelihood: given sample에 대해 각 클래스가 나올 확률 Likelihood.}
% \jw{적으면서 보니까, 광무형이 보내셨던 식 derivation에 조금 오류가 있습니다.
% $P(Y|X,Y’) P(X|Y’)P(Y’)/P(X)= P(Y,X|Y’)/P(X) P(X|Y’)P(Y’)/P(X)$ 가 아니라 $P(Y|X,Y’) P(X|Y’)P(Y’)/P(X)= P(Y,X|Y’)P(Y')/P(X,Y') P(X|Y’)P(Y’)/P(X)=P(Y,X|Y’)P(Y')/P(X,Y') P(X,Y')/P(Y') P(Y’)/P(X)=P(Y,X|Y’)P(Y')/P(X)$로 derive됩니다. 이러면 X에 대해 marginalization시키면 X에 대한 term이 분모의 prior밖에 남지 않아서 likelihood가 배제되게 됩니다.
% 일단 광무형이 마지막에 제안하신 X, Y가 sampling 되기 전에는 의미 없으니 제거한다는 내용을 기반으로 각 unlabel sample은 아직 label이 없어 real label이 될 확률이 uniform하다 해버리고 없애는 것으로 적어보았습니다. 이 부분은 계속 논의를 좀 해야할 것 같습니다.
% }

Then, we estimate each of the three terms by using the variational classification results from the trained VAE.
At first, the label uncertainty can be estimated by using the labeled samples of $\calP_c$ that is excluded when the VAE is trained. Thus,
\begin{equation}\label{eq:labelUncertaintyProb}
    P(\by_n | \widehat{\by}_n) = \frac{ \sum_{l\in L, (\bx_c^{(i)},\by_c^{(i)})\in \calP_c} \delta (\widehat{\by}^{(i,l)}, \by_c^{(i)}, n)}{\sum_{l\in L, (\bx_c^{(i)},\by_c^{(i)})\in \calP_c} \delta (\widehat{\by}^{(i,l)}, n)}
\end{equation}
where $\delta(\bullet)$ is a function resulting $1$ if all the inputs are equivalent otherwise $0$, and $L$ is a set containing the latent noises. The size of $L$ is determined by a user-defined parameter $N_L$.

Next, the likelihood is estimated for each unlabeled sample of $\mathcal{P_o}$ as following:
\begin{equation}\label{eq:likelihood}
    P(\bx_o^{(i)} | \widehat{\by}_n) = \frac{\sum_{l\in L} \delta ( \widehat{\by}^{(i,l)}, n)}{N_L}.
\end{equation}

At last, the prior is acquired by using the unlabeled samples included in $\mathcal{P_o}$.
Thus,
\begin{equation}\label{eq:prior}
    P(\widehat{\by}_n) = \frac{\sum_{l\in L, \bx_o^{(i)}\in \calP^o} \delta (\widehat{\by}^{(i,l)}, n)}{N_L N(\calP^o)},
\end{equation}
where $N(\bullet)$ means the number of elements in the given pool.

Then, we can estimate the posterior uncertainty $P( \by \neq \widehat{\by} | \bx )$ for every sample according to Eq.~\ref{eq:posteriorUncertainty}.
Then, the labeling query is found by selecting the $N_s$ samples with the highest posterior uncertainty as:
\begin{equation}
    Q = \arg \max_{\bx\in\calP_o}\,_{N_s} P( \by \neq \widehat{\by} | \bx ),
\end{equation}
where $\max\,_{N_s}(\bullet)$ results in the $N_s$ maximum values of the input vectors.\jw{??}
%Among all the samples in the unlabeled pool, we select the samples with the highest posterior uncertainty to be labeled for the next sampling step.


